Incentivized Exploration via Filtered Posterior Sampling

We study "incentivized exploration" (IE) in social learning problems where the principal (a recommendation algorithm) can leverage information asymmetry to incentivize sequentially-arriving agents to take exploratory actions. We identify posterior sampling, an algorithmic approach that is well known in the multi-armed bandits literature, as a general-purpose solution for IE. In particular, we expand the existing scope of IE in several practically-relevant dimensions, from private agent types to informative recommendations to correlated Bayesian priors. We obtain a general analysis of posterior sampling in IE which allows us to subsume these extended settings as corollaries, while also recovering existing results as special cases.

==> Technical_stuff.tex <==











%\section{Addendum: notes on linear models}

% \subsection{Some notes on TS for K-armed bandits}

% Relative to extant literature on incentivized exploration (IE) in bandit problems (\cite{mansour2020bayesian, immorlica2018incentivizing}), and more specifically on IE via Thompson Sampling (\cite{sellke2021price, hu2022incentivizing, sellke2023incentivizing}), Theorem~1 contributes along two dimensions: (i) The message space is expanded to rank-order-lists (ROL) from single arm recommendations. ROL is a natural and well-motivated message space that is routinely encountered in applications such as Yelp, WebMD, Netflix, etc., that display an ordered list of suggestions to visiting users based on relevance to their profile or an explicit keyword query. In applications like Yelp and WebMD, in addition, the platform may at the time of listing recommendations be unaware of which options are actually available at that time. For instance, a recommended restaurant may not currently have any available spots,  or the top medical provider on the list may not be taking new admissions temporarily.  This may lead to \emph{sleeping bandits}-esque situations where users may be forced to choose down the list owing to infeasibility of top suggestions, and for that reason, it is important that the ordered list is ``smartly'' curated.  In terms of technical analysis, generalization to ranked lists is non-trivial as standard proof recipes for single arm recommendations, e.g., the FKG (or Harris) inequality and martingale-based approach in \cite{sellke2021price,hu2022incentivizing}, fail to generalize to complex message spaces like ranked lists on account of failure of key monotonicity properties.  \akcomment{Additional information can exacerbate the situation; see Example~\ref{example} below} (ii) Case of correlated priors: All extant works (barring \cite{sellke2023incentivizing} and a result for $K=2$ in \cite{hu2022incentivizing}) posit a product-form (independent) prior over the $K$ arms. Theorem~\ref{thm:general} extends this line of results to allow for arbitrary correlations across arms.

% \begin{example}
% \label{example}
% Consider i.i.d. $\trueModel_1,\trueModel_2,\trueModel_3\sim\text{Uniform}([0,1])$. Define $\Delta_1 := \bb{E}\left[ \trueModel_1 - \trueModel_2 | \trueModel_1 > \max(\trueModel_2, \trueModel_3) \right]$ and $\Delta_2 := \bb{E}\left[ \trueModel_1 - \trueModel_2 |  \trueModel_1 > \trueModel_2 > \trueModel_3 \right]$. Then, note that $\Delta_1 = 3/8 > 1/4 = \Delta_2$.
% \end{example}

%\subsection{Some notes on linear models}

% \textbf{Regret.} The ex post regret of mechanism $\pi$ after $T$ rounds is given by
% \begin{align}
% \texttt{Regret}^\pi(\trueModel, T) := \bb{E}\left[ \left. \sum_{t\in[T]} \max_{k\in\cal{K}}x_k(t)\cdot\trueModel \right\rvert \trueModel \right] - \bb{E}\left[ \left. \sum_{t\in[T]} x_{A_t^\pi}(t)\cdot\trueModel \right\rvert \trueModel  \right], \label{eqn:regret}
% \end{align}
% where $\bb{E}\left[ \left. \sum_{t\in[T]} \max_{k\in\cal{K}}x_k(t)\cdot\trueModel \right\rvert \trueModel \right]$ is the ``ex post first-best,'' $A_t^\pi\in\Delta(\cal{K})$ is the arm played by agent $t$ under mechanism $\pi$, and the expectations are w.r.t. all the sources of randomness in the problem (minus the prior $\cal{P}_0$). The Bayesian regret (or risk) defined w.r.t. the prior $\cal{P}_0$ is given by 
% \begin{align}
% \texttt{Bayes-regret}^\pi(T) := \E_0\left[ \texttt{Regret}^\pi(\trueModel,T) \right]. \label{eqn:regret-bayes}
% \end{align}



% \begin{assumption}[Covariate diversity]
% \label{assumption:diversity}
% The context distribution $\cal{D}$ satisfies
% \begin{align}
% \lambda_{\min}\left( \bb{E}_{\left( x_1, ..., x_K \right)\sim\cal{D}} \left[ \frac{1}{K}\sum_{k\in[K]}x_kx_k\cdot \right] \right) =: \lambda_0 > 0. \label{eqn:diversity}
% \end{align}
% \end{assumption}
% This is a fairly innocuous assumption that has been popular in the contextual bandit literature and appeared, e.g., as ``diversity outside margin'' and related conditions in  \cite{goldenshluger2013linear,bastani2020online,hamidi2020general,bastani2021mostly,gur2022smoothness}, and as ``context smoothing'' in \cite{kannan2018smoothed,sivakumar2020structured,raghavan2023greedy}, among others. It has also appeared in the automatic control and system identification literature as ``persistence of excitation'' (see, e.g., \cite{goldenshluger2011note}). Note that Assumption~\ref{assumption:diversity} appeared as is in \cite{li2017provably} which is the mildest among all versions appearing in aforementioned papers.



% \begin{lemma}[$\cal{O}\left( \log T \right)$ random samples suffice for spectral diversity]
% \label{lemma:warm-start}
% Suppose that Assumption~\ref{assumption:diversity} holds. Let $\hat{\Sigma}_t := \cal{I} + \sum_{s\in[t-1]}x_{A_s, s}x_{A_s, s}\cdot$ denote the empirical covariance matrix after $t-1$ rounds of ``uniform exploration,'' i.e., $\bb{P}(A_s=k)=1/K\ \forall\ k\in\cal{K},\ s\in\bb{N}$ independently. For some hyperparameters $b_1,b_2>0$, define $\tau := \inf \left\lbrace t\in\bb{N} : \lambda_{\min}\left( \hat{\Sigma}_t \right) \geqslant b_1\log \left(b_2T\right) \right\rbrace$. Then,
% \begin{align*}
% \bb{E}\left[ \tau\wedge T \right] \leqslant \left( \frac{C_1\sqrt{d} + C_2\sqrt{\log T}}{\lambda_0} \right)^2 + \frac{2b_1\log \left(b_2T\right)}{\lambda_0} + C_3,
% \end{align*}
% where $\lambda_0$ is as defined in \eqref{eqn:diversity} and $C_1,C_2,C_3>0$ are universal constants.
% \end{lemma}

% \subsubsection{Proof of Lemma~\ref{lemma:warm-start}} 


% Note that $\hat{\Sigma}_t = \cal{I} + \tilde{\Sigma}_{t-1}$, where $ \tilde{\Sigma}_{t-1}$ satisfies the conditions of Fact~\ref{fact:vershynin}. 
% Then,
% \begin{align*}
% \bb{E}\left[ \tau\wedge T\right] \leqslant \sum_{t=1}^{T}\bb{P}\left( \tau \geqslant t \right) &= 1 + \sum_{t=2}^{T}\bb{P}\left( \cap_{s\in[t-1]} \left\lbrace  \lambda_{\min}\left( \hat{\Sigma}_s \right) < b_1\log \left(b_2T\right) \right\rbrace \right) \\
% &\leqslant 1 + \sum_{t=1}^{T}\bb{P}\left( \lambda_{\min}\left( \hat{\Sigma}_{t} \right) < b_1\log \left(b_2T\right) \right) \\
% &\leqslant 1 + \sum_{t=1}^{T}\bb{P}\left( \lambda_{\min}\left( \tilde{\Sigma}_{t-1} \right) < b_1\log \left(b_2T\right) \right) \\
% &\leqslant 2 + \sum_{t=1}^{T}\bb{P}\left( \lambda_{\min}\left( \tilde{\Sigma}_{t} \right) < b_1\log \left(b_2T\right) \right) \\
% &\leqslant 2 + \sum_{t=1}^{T}\mathbbm{1}\left\lbrace f(t) < b_1\log \left(b_2T\right)) \right\rbrace + \delta^\prime T,
% \end{align*}
% where $f(t) := \lambda_0 t - C_1\sqrt{dt} - C_2\sqrt{t\log(1/\delta^\prime)}$ (by Fact~\ref{fact:vershynin}).  For $\delta^\prime = 1/T$, note that $f(t) \geqslant b_1\log \left(b_2T\right)$ for $t \geqslant \left( \frac{C_1\sqrt{d} + C_2\sqrt{\log T}}{\lambda_0} \right)^2 + \frac{2b_1\log \left(b_2T\right)}{\lambda_0}$. Therefore,
% \begin{align*}
% \bb{E}\left[ \tau\wedge T \right] \leqslant \left( \frac{C_1\sqrt{d} + C_2\sqrt{\log T}}{\lambda_0} \right)^2 + \frac{2b_1\log \left(b_2T\right)}{\lambda_0} + C_3,
% \end{align*}
% where $C_1,C_2,C_3>0$ are universal constants. \hfill $\square$
